MNL-Bandit with Knapsacks: a near-optimal algorithm

We consider a dynamic assortment selection problem where a seller has a fixed inventory of $N$ substitutable products and faces an unknown demand that arrives sequentially over $T$ periods. In each period, the seller needs to decide on the assortment of products (satisfying certain constraints) to offer to the customers. The customer's response follows an unknown multinomial logit model (MNL) with parameter $\boldsymbol{v}$. If customer selects product $i \in [N]$, the seller receives revenue $r_i$. The goal of the seller is to maximize the total expected revenue from the $T$ customers given the fixed initial inventory of $N$ products. We present MNLwK-UCB, a UCB-based algorithm and characterize its regret under different regimes of inventory size. We show that when the inventory size grows quasi-linearly in time, MNLwK-UCB achieves a $\tilde{O}(N + \sqrt{NT})$ regret bound. We also show that for a smaller inventory (with growth $\sim T^{\alpha}$, $\alpha < 1$), MNLwK-UCB achieves a $\tilde{O}(N(1 + T^{\frac{1 - \alpha}{2}}) + \sqrt{NT})$. In particular, over a long time horizon $T$, the rate $\tilde{O}(\sqrt{NT})$ is always achieved regardless of the constraints and the size of the inventory.

==> conclusion.tex <==
\section{Conclusion}

In this paper, we study a dynamic assortment selection problem under an unknown MNL demand and inventory constraints. We propose an optimistic algorithm which achieves near-optimal regret $\tilde O(\sqrt{T})$ in the large-inventory setting. Our algorithm involves repeatedly solving an exponentially sized LP, which we prove to be tractable by presenting an approximation algorithm based on a difference of MNL assortment optimization problem. Our results are thus significantly stronger than \cite{Cheung_assort_inventory}, which presents an algorithm that incurs a $\tilde O(T^{2/3})$ regret and an intractable algorithm with a  $\tilde O(\sqrt{T})$ regret.

Even though solving the LP can be done in polynomial time, this is still a computationally expensive step. Motivated by recent algorithms based on online convex optimization for the online allocation framework \cite{lu2020dual}, one interesting research direction would be to study whether faster algorithms can be obtained in our setting while still achieving the same regret bounds. 
